Exploiting Longitudinal Speech Sessions via Voice Assistant Systems for Early Detection of Cognitive Decline

Mild Cognitive Impairment (MCI) is an early stage of Alzheimer's disease (AD), a form of neurodegenerative disorder. Early identification of MCI is crucial for delaying its progression through timely interventions. Existing research has demonstrated the feasibility of detecting MCI using speech collected from clinical interviews or digital devices. However, these approaches typically analyze data collected at limited time points, limiting their ability to identify cognitive changes over time. This paper presents a longitudinal study using voice assistant systems (VAS) to remotely collect seven-session speech data at three-month intervals across 18 months. We propose two methods to improve MCI detection and the prediction of cognitive changes. The first method incorporates historical data, while the second predicts cognitive changes at two time points. Our results indicate improvements when incorporating historical data: the average F1-score for MCI detection improves from 58.6% to 71.2% (by 12.6%) in the case of acoustic features and from 62.1% to 75.1% (by 13.0%) in the case of linguistic features. Additionally, the prediction of cognitive changes achieves an F1-score of 73.7% in the case of acoustic features. These results confirm the potential of VAS-based speech sessions for early detection of cognitive decline.

==> 5_Discussion.tex <==
\section{Conclusion and Future Work} 
This paper demonstrates the use of spontaneous speech data collected from VAS for early detection and monitoring of MCI changes. We found that both acoustic and linguistic features, extracted using pre-trained models, are important in identifying speech patterns directly linked to MCI. Additionally, our work employed two methods for analyzing longitudinal data: predicting cognitive status (MCI or healthy control) in future events and predicting cognitive changes over time. We focused on utilizing historical and sequential data to enhance prediction performance and overcome the issues associated with small data sizes and data imbalances. 

However, this work has some limitations, including a small participant group and reliance on pre-trained models for extracting features. Additionally, we didn't explore how individual questions contribute to identifying cognitive changes. Future work will aim to overcome these limitations, expand our dataset, and investigate more disease-related features to refine MCI detection and long-term monitoring.




% \section{Ethical Statement}
% The study was supported by [invisible in the review process] and data for this study were collected by [invisible in the review process] in compliance with regulations in involved institutions. The [invisible in the review process] approved using this data for research purposes. All participants' written informed consent was obtained. Additionally, the data analysis ensured the exclusion of any personally identifiable information.
